Translating Hanja Historical Documents to Contemporary Korean and English

The Annals of Joseon Dynasty (AJD) contain the daily records of the Kings of Joseon, the 500-year kingdom preceding the modern nation of Korea. The Annals were originally written in an archaic Korean writing system, `Hanja', and were translated into Korean from 1968 to 1993. The resulting translation was however too literal and contained many archaic Korean words; thus, a new expert translation effort began in 2012. Since then, the records of only one king have been completed in a decade. In parallel, expert translators are working on English translation, also at a slow pace and produced only one king's records in English so far. Thus, we propose H2KE, a neural machine translation model, that translates historical documents in Hanja to more easily understandable Korean and to English. Built on top of multilingual neural machine translation, H2KE learns to translate a historical document written in Hanja, from both a full dataset of outdated Korean translation and a small dataset of more recently translated contemporary Korean and English. We compare our method against two baselines: a recent model that simultaneously learns to restore and translate Hanja historical document and a Transformer based model trained only on newly translated corpora. The experiments reveal that our method significantly outperforms the baselines in terms of BLEU scores for both contemporary Korean and English translations. We further conduct extensive human evaluation which shows that our translation is preferred over the original expert translations by both experts and non-expert Korean speakers.

==> contents/dataset.tex <==
\begin{table*}[t]
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{l|c|M{1.25cm}M{1.25cm}M{1.25cm}M{1.25cm}|M{1.3cm}|r}
\toprule
 \textbf{Annals of} & \textbf{Reign} & \textbf{Hanja} & \textbf{original Korean} & \textbf{new Korean} & \textbf{English} & \textbf{\# of sentences}& \multicolumn{1}{c}{\textbf{Ratio}(\%)}\\
\midrule 
\textbf{Joseon Dynasty}& 1392-1910 & \Circle & \Circle &         & & \multicolumn{1}{r|}{359,726} & 100.0 \\
\textbf{22\textsuperscript{th} King Jeongjo}&1776-1799& \Circle & \Circle & \Circle & & \multicolumn{1}{r|}{14,356}  & 3.9 \\
\textbf{4\textsuperscript{th} King Sejong}&1418-1449& \Circle & \Circle &  & \Circle & \multicolumn{1}{r|}{26,227} & 7.2 \\
\bottomrule
\end{tabular}
\caption{
Statistics of our dataset. 
For the entire AJD, there are \textlangle{}Hanja, original Korean\textrangle{} pairs.
The Annals of King Jeongjo and Annals of King Sejong are the subset of the Annals of Joseon Dynasty and but the new Korean or English translation only exist for that part. The ratio is the portion of each data on the basis of the total AJD.
}
\label{tab:dataset}
\end{table*}

% The Annals of the Joseon Dynasty (AJD), also called the Veritable Records of the Joseon Dynasty, is a corpus of 27 sets of chronological records, and each set covers one ruler’s reign. 
\emph{The Annals of the Joseon Dynasty} (AJD), also called \emph{the Veritable Records of the Joseon Dynasty}, is an old and vast volume of historical document of Korea.
It records the 472 years (1392 - 1863) of the 25 rulers' reigns of Joseon Dynasty in chronological order.
It covers historical facts in various fields and has high integrity and credibility in describing history, making it invaluable as a historical record.\footnote{The description for AJD is based on Korean Cultural Heritage Administration (\url{https://www.cha.go.kr/}).}
The dataset is available at the website\footnote{Website for `The Veritable Records of the Joseon Dynasty' \url{http://sillok.history.go.kr/}} guided by National Institute of Korean History (NIKH).
AJD was originally written in Hanja, the writing system of ancient Korea, consists of totally different characters and syntactic structure from Korean.
Hanja had stemmed from traditional Chinese, but the lexical, semantic, and syntactic characteristics had changed to reflect the cultural differences between the Joseon and ancient China.

AJD was translated from Hanja to Korean during 1968 - 1993, and the dataset is uploaded on the website\footnote{Both the original translation of AJD and the new translation of AKJ are available at \url{https://db.itkc.or.kr/}.} of the Institute for the Translation of Korean Classics (ITKC).
% However, as in Table \ref{table:ex_data}, the original translation is a literal translation, including many unused words and using Hanja-style writing.
The original translations include numerous outdated Hanja words which contemporary Korean native speakers cannot understand and semantic errors not considering historical contexts.
To correct those errors and improve readability of the original translation, ITKC has launched project for modernizing translation of AJD since 2011.
\emph{The Annals of the 22nd King Jeongjo} (AKJ) was first newly translated\footnotemark[3] from 2012 to 2016.
Throughout this paper, we will refer to the original translation as oKo, and the new translation as nKo.


% 국사편찬위원회의 조선왕조실록 영문판 보급사업은 2011년 기초조사를 거쳐 2012년 처음으로 사업이 시작되었다.
% 조선왕조실록 영문판 보급사업은 조선왕조실록을 전 세계에 보급하여 국외에서의 한국사 및 동아시아사 연구에 기여하고, 우리 역사에 관심이 있는 외국의 일반 독자들에게 한국을 알리며, 나아가 세계인들의 기록문화유산이라는 그 위상에 걸맞도록 인류문명의 발전에 기여할 수 있도록 하는 것을 궁극적인 목표로 한다.
% 이러한 경험을 바탕으로 2013년부터 세종실록 즉위년 이래의 원문 기사를 본격적으로 번역하면서 매년 그 분량을 늘려가고 있다.
For the globalization of AJD, listed as UNESCO's Memory of the World, and Korean history, NIKH has been translating AJD into English.
\emph{The Annals of the 4th King Sejong} (AKS) has been being translated first since 2013, and the dataset is released at the website\footnote{The English translation of AJD is available at \url{http://esillok.history.go.kr/}.}.
These translation projects are expected to take two more decades.

Table \ref{tab:dataset} represents the statistics of the datasets.
There are only a few amounts of training corpora for new Korean or English translations compared to the Hanja and original Korean pairs. 
